A practical key-recovery attack on LWE-based key-encapsulation mechanism schemes using Rowhammer

Physical attacks are serious threats to cryptosystems deployed in the real world. In this work, we propose a microarchitectural end-to-end attack methodology on generic lattice-based post-quantum key encapsulation mechanisms to recover the long-term secret key. Our attack targets a critical component of a Fujisaki-Okamoto transform that is used in the construction of almost all lattice-based key encapsulation mechanisms. We demonstrate our attack model on practical schemes such as Kyber and Saber by using Rowhammer. We show that our attack is highly practical and imposes little preconditions on the attacker to succeed. As an additional contribution, we propose an improved version of the plaintext checking oracle, which is used by almost all physical attack strategies on lattice-based key-encapsulation mechanisms. Our improvement reduces the number of queries to the plaintext checking oracle by as much as $39\%$ for Saber and approximately $23\%$ for Kyber768. This can be of independent interest and can also be used to reduce the complexity of other attacks.

==> Images/BST_v.tex <==
\begin{figure}[!ht]
	\centering
	\scalebox{.5}{
		\begin{tikzpicture}
	%		\node[font=\Huge](a) at (5.7,10){${\bf s}[j]\in S_{0}$};
			\node[ font=\Huge,rectangle, draw, minimum size=1cm] (a) at (5.7,8.8) {$d_{0}$};
	%		\node[font=\Huge](b) at (0,6.8){${\bf s}[j]\in S_{1}$};
	%		\node[font=\Huge](b) at (11,6.8){${\bf s}[j]\in S_{2}$};
			\draw[font=\Huge][blue,->](5.7,8.3) -- (0,6.6)node[midway,above]{{\tt O} };
			\draw[font=\Huge][red,->](5.7,8.3) -- (11,6.6)node[midway,above]{{\tt 1} };
			\node[font=\Huge ,rectangle, draw,minimum size=1cm] (a) at (11,6) {$d_{2}$};
			%\node[font=\Huge](b) at (9,3.1){${\bf s}[j]\in S_{5}$};
			%\node[font=\Huge](b) at (13,3.1){${\bf s}[j]\in S_{6}$};
		%	\draw[font=\Huge][blue,->](11,5.1) -- (9,3.6)node[midway,above]{{\tt O} };
		%	\draw[font=\Huge][red,->](11,5.1) -- (13,3.6)node[midway,above]{{\tt 1} };
			\node[font=\Huge, rectangle, draw,minimum size=1cm] (c) at (0,6) {$d_{1}$};
			%\node[font=\Huge](b) at (-2,3.1){${\bf s}[j]\in S_{3}$};
			%\node[font=\Huge](b) at (2,3.1){${\bf s}[j]\in S_{4}$};
			\draw[font=\Huge][blue,->](0,5.5) -- (-2,3.6)node[midway,above]{{\tt O} };
			\draw[font=\Huge][red,->](0,5.5) -- (2,3.6)node[midway,above]{{\tt 1} };
			\node[ font=\Huge ,rectangle, draw,minimum size=1cm] (a) at (2,3) {$d_{4}$};
		%	\node[ font=\Huge](c) at (0,-0.5){${\bf s}[j]\in S_{9}$};
		%	\node[ font=\Huge](c) at (4,-0.5){${\bf s}[j]\in S_{10}$};
		%	\draw[ font=\Huge][blue,->](2,1.4) -- (0,0)node[midway,above]{{\tt O} };
		%	\draw[ font=\Huge][red,->](2,1.4) -- (4,0)node[midway,above]{{\tt 1} };
            \node[ font=\Huge](c) at (10,-0.5){$..........$};
            \node[ font=\Huge](c) at (3,-2){$..........$};
		\end{tikzpicture}
	}
	\caption{Binary tree to select the value of $k_{v_{j}}=d_{i}$ for each $v[j]$}
	\label{generic}
\end{figure}

==> Images/Kyber-decaps.tex <==
\begin{figure}[H]
     \centering
\setlength{\nodedistance}{4mm}
% \resizebox{width=\linewidth}{!}{%
\begin{tikzpicture}[ % <--- used style are moved here 
node distance = \nodedistance,
operation/.style = {circle, draw=black},
bigoperation/.style = {rounded corners, draw=black},
operationsecret/.style = {circle, draw=black, fill=black!20!white, text=black},
bigoperationsecret/.style = {rounded corners, draw=black, fill=black!20!white, text=black},
operant/.style = {},
halfblockdraw/.style = {draw, rounded corners},
     line/.style = {draw, -Latex}
                       ]
% Place nodes
% bp * s
\node (multbps) [bigoperationsecret]  {$\mathtt{Decomp}$};
\node (bp) [operant, left=of multbps.west]  {$\pmb{u}$};
\draw[->] (bp) -- (multbps);

% \node (s) [operant, above=of multbps.north]  {$\pmb{s}$};
% \draw[->] (s) -- (multbps);

% v + h addition
\node (addvh) [operationsecret, right=of multbps]  {X};
\draw[->] (multbps.east) -- (addvh.west);
\node (h2) [operant, above=of addvh.north]  {$\pmb{s}$};
\draw[->] (h2) -- (addvh);

% cm
\node (cm) [operant, below=of bp]  {$v$};
\node (shiftcm) [bigoperationsecret, right=of cm]  {$\mathtt{Decomp}$};
\draw[->] (cm) -- (shiftcm);

% % cm - v
% \coordinate [right=of addvh](addvhright);
% \node (subcmv) [operationsecret] at (addvhright |- shiftcm) {$-$};
% \draw[->] (addvh) -- (addvhright) -- (subcmv);
% \draw[->] (shiftcm) -- (subcmv);

% cm - v
\node (subcmv) [operationsecret, right = of shiftcm ] {$-$};
\draw[->] (addvh) -- (subcmv);
\draw[->] (shiftcm) -- (subcmv);

% Tobin
\node (tobin) [bigoperationsecret, right=of subcmv]  {$\mathtt{Compress}$};
\draw[->] (subcmv) -- (tobin);

\node[draw=blue, dashed, thick, fit=(h2) (shiftcm) (tobin)](ciphertext) {};

% G(pk, m)
\node (g) [bigoperationsecret, right=of tobin]  {$\mathcal{G}$};
\coordinate  (m) at ($(tobin.east)!0.5!(g.west)$);
\node (pkh) [operant, above=of g]  {$\mathcal{H}(pk)$};
\draw[->] (pkh) -- (g);
\draw[->] (tobin) -- (g);

\node (K) [operant, below=of g]  {$K'$};
\draw[->] (g) -- (K);

% gen secret
\node (beta1) [bigoperationsecret, right=of g]  {Enc};
\draw[->] (g) -- (beta1);

% add m
\coordinate [below=0.5\nodedistance of K](tmp); 
\draw[->] (m) -- (m |- tmp) -- (beta1 |- tmp) -- (beta1);

\node (beta2) [operant, right=of beta1]  {$c=(\pmb{u}'_*, {v}_{m*})$};
\draw[->] (beta1) -- (beta2);

% compare
\node[draw=black, dotted, thick, fit=(beta2)](ciphertext2) {};
\node[draw=black, dotted, thick, fit=(bp) (cm)](ciphertext) {};
\coordinate [below=1.5\nodedistance of K](x); 
\coordinate (y) at ($(ciphertext)!0.5!(ciphertext2)$);
\node (comp) [operationsecret] at (y |- x)  {$=?$};

\draw[->] (ciphertext) -- (ciphertext |- x) -- (comp);
\draw[->] (ciphertext2) -- (ciphertext2 |- x) -- (comp);

% Two results
\node (correct) [bigoperation, below left=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{F}(K', ct)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below left=0.5\nodedistance and 1.3\nodedistance of comp] (yes) {yes};

\node (correct) [bigoperation, below right=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{F}(z, ct)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below right=0.5\nodedistance and 1.3\nodedistance of comp] (no) {no};
\end{tikzpicture}
%}

\caption{Decapsulation algorithm of KEM of CRYSTALS-KYBER/SABER. The components inside the blue dashed rectangle represent the decryption part of the decapsulation algorithm.}
\label{fig:KyberDecap}
\end{figure}

==> Images/SecretTree.tex <==
\begin{figure}[!ht]
	\centering
	\scalebox{.5}{
		\begin{tikzpicture}
			\node[font=\Huge](a) at (5.7,10){${\bf s}[j]\in S_{0}$};
		%	\node[ font=\Huge,rectangle, draw, minimum size=1cm] (a) at (5.7,8.8) {$d_{0}$};
			\node[font=\Huge](b) at (0,6.8){${\bf s}[j]\in S_{1}$};
			\node[font=\Huge](b) at (11,6.8){${\bf s}[j]\in S_{2}$};
			\draw[font=\Huge][blue,->](5.7,8.3) -- (0,7.2)node[midway,above]{{\tt O} };
			\draw[font=\Huge][red,->](5.7,8.3) -- (11,7.2)node[midway,above]{{\tt 1} };
		%	\node[font=\Huge ,rectangle, draw,minimum size=1cm] (a) at (11,5.6) {$d_{2}$};
			\node[font=\Huge](b) at (9,3.1){${\bf s}[j]\in S_{5}$};
			\node[font=\Huge](b) at (13,3.1){${\bf s}[j]\in S_{6}$};
			\draw[font=\Huge][blue,->](11,5.1) -- (9,3.6)node[midway,above]{{\tt O} };
			\draw[font=\Huge][red,->](11,5.1) -- (13,3.6)node[midway,above]{{\tt 1} };
		%	\node[font=\Huge, rectangle, draw,minimum size=1cm] (c) at (0,5.6) {$d_{1}$};
			\node[font=\Huge](b) at (-2,3.1){${\bf s}[j]\in S_{3}$};
			\node[font=\Huge](b) at (2,3.1){${\bf s}[j]\in S_{4}$};
			\draw[font=\Huge][blue,->](0,5.1) -- (-2,3.6)node[midway,above]{{\tt O} };
			\draw[font=\Huge][red,->](0,5.1) -- (2,3.6)node[midway,above]{{\tt 1} };
		%	\node[ font=\Huge ,rectangle, draw,minimum size=1cm] (a) at (2,1.9) {$d_{4}$};
			\node[ font=\Huge](c) at (0,-0.5){${\bf s}[j]\in S_{9}$};
			\node[ font=\Huge](c) at (4,-0.5){${\bf s}[j]\in S_{10}$};
			\draw[ font=\Huge][blue,->](2,1.4) -- (0,0)node[midway,above]{{\tt O} };
			\draw[ font=\Huge][red,->](2,1.4) -- (4,0)node[midway,above]{{\tt 1} };
            \node[ font=\Huge](c) at (10,-0.5){$..........$};
            \node[ font=\Huge](c) at (3,-2){$..........$};
		\end{tikzpicture}
	}
	\caption{Binary tree to select the value of $k_{v_{j}}=d_{i}$ for each $v[j]$}
	\label{generic}
\end{figure}

==> Sections/RelatedWorks.tex <==
\section{Related Works}

Lattice-based post-quantum KEMs are vulnerable to side-channel attacks. A timing attack on the \texttt{KEM.Decaps} has been shown in~\cite{TimingPQC}, it targets the non-constant time implementation of the ciphertext equality checking (Line 4 in \texttt{KEM.Decap} algorithm of Figure~\ref{fig:fo-kem}). \cite{Sidechannelattacks1}, proposed a generic and practical  Electromagnetic (EM) power analysis assisted CCA on LWE-based KEMs. They also target the \texttt{KEM.Decaps} in their attack. They have constructed a plaintext-checking oracle $\mathcal{O}$ with the help of an EM power attack, which can distinguish two particular messages. This message provides single-bit information related to one coefficient of the secret key. Continuing the same methods, the attacker can find the whole secret key. This paper has shown that $2000$ to $4000$ queries are required to retrieve the complete secret key for Kyber. \cite{ParallelPC} reduced the query requirements by creating a multiple-valued plaintext-checking oracle. Here, the attacker acquires information regarding multiple secret key coefficients from a single query. In~\cite{ParallelPC1}, the authors further reduced the number of queries required to recover the whole secret keys by improving the model of plaintext-checking oracle. One significant area of research in this domain revolves around improving the efficiency of attacks by minimizing the number of required quires. This reduction enables a more precise evaluation of the cost of an optimal attack. Our attack contributes in this direction.




As the first $t$ message bits are directly linked to their corresponding secret coefficients, the attacker acquires $t$ bits of information of the coefficients $\Bar{\bf s}{0}[0], \dots, \Bar{\bf s}{0}[t-1]$ using the decrypted message $m$. 



In the paper \cite{ParallelPC}, the authors present side-channel attacks on post-quantum KEMs CRYSTAL KYBER \cite{KYBER}, SABER \cite{SABER}, FRODO \cite{FRODO}, NTRU Prime, as well as SIKE \cite{SIKE} by creating multiple-valued plaintext-checking oracle. These schemes had selected candidates in the NIST standardization process, and CRYSTAL KYBER has been selected as the winner. The authors demonstrate very efficient strategies to make $\mu$ plaintexts checking oracle $\mathcal{O}_{\mu}$ as follows:


% applicable to six IND-CCA secure LWE/LWR-based PKE/KEMs. These schemes were the candidates in the NIST standardization process. They demonstrate very efficient strategies to instantiate the EM side-channel as two particular plaintexts checking oracle $\mathcal{O}$ as follows:

% In \cite{TimingPQC}, the authors present a timing attack on the algorithm KEM\\\_Decaps() (Algo \ref{KEM_Decap}) and target the equality checking process (line no: 4). Since the ciphertexts of these post-quantum schemes are large, the comparison test of two ciphertexts $ct$ and $c$ takes more time if they are almost similar or similar; otherwise it will take less time. The authors can find the secret key from the leakage of this timing attack. \\

% In the paper \cite{FRODOFLIP}, the authors focus on the FrodoKEM algorithm\cite{FRODO}. The FrodoKEM algorithm is being considered for standardization by NIST in their Post Quantum Cryptography (PQC) process.
% The authors propose a new method to recover the private key material used in the FrodoKEM key exchange mechanism. They achieve this by exploiting a hardware-based security vulnerability Rowhammer.
% The authors use the Rowhammer vulnerability to manipulate the FrodoKEM Key Generation (KeyGen) process. By repeatedly accessing specific memory rows, they induce the FrodoKEM software to output a higher-error Public Key $(PK)$, denoted as $(A, B = AS + E)$. The error term $E$, which affects the algorithm's security, is modified through the rowhammer attack.
% This research demonstrates an approach to exploiting the FrodoKEM algorithm's vulnerability to rowhammer and recovering private key material. These findings have implications for the security of the FrodoKEM algorithm.\\

In the subsequent section, we elucidate the binary plaintext checking (PC) oracle attack on Kyber KEM, as presented by~\cite{Sidechannelattacks1} and the parallel PC oracle attack on Kyber KEM which is presented by ~\cite{ParallelPC1}. These attacks form the foundation of our enhanced strategies.

\subsection{Binary PC oracle on Kyber KEM}
By employing a coefficient-by-coefficient approach, the attack successfully retrieves the secret key. Thus, we showcase the recovery of a specific coefficient, $\Bar{{\bf s}}_{0}[0]$, while employing a similar methodology to recover the remaining coefficients.

To find the secret coefficient $\Bar{\bf s}_{0} [0]$,
the attacker constructs the dummy ciphertext $c = (\Bar{\bf u}, {\bf v})$ where $\Bar{\bf u}_{0} [0] = k_{u}$ and $ {\bf v}[0] = k_{v} $ are non zero and
others coefficients of $\Bar{\bf u}$ and ${\bf v}$ are zero.
Then the decrypted message $m$ will be
\begin{equation}
m^{j}=
    \begin{cases}
        \text{Decode}(k_{v} - k_{u}\Bar{\bf s}_{0}[0]) & \text{if } j=0\\
         \text{Decode}( - k_{u}\Bar{\bf s}_{0}[j]) & \text{if } 1\leq j \leq n-1
    \end{cases}    
\end{equation}

From the previous computation, it is clear that the $j^{th}$ bit of the decrypted message $m$ depends on the corresponding secret coefficient $\Bar{\bf s}_{0}[j]$ and the values of $k_{u}$ and $k_{v}$. The attacker chooses the values of $k_{u}$ and $k_{v}$ such that 
$ \text{Decode}( - k_{u}\Bar{\bf s}_{0}[j])$ will be zero for any secret coefficient $\Bar{\bf s}_{0}[j]$ and the $0^{th}$ bit of message $m$ only depends on the secret coefficient $\Bar{\bf s}_{0}[0]$. i.e.,
\begin{equation}
m^{j}=
    \begin{cases}
        \text{Decode}(k_{v} - k_{u}\Bar{\bf s}_{0}[0]) & \text{if } j=0\\
        0 & \text{if } 1\leq j\leq n-1
    \end{cases}    
\end{equation}.
so, the decrypted message $m$ will be either $\mathbb{0}$ (all bits are zero) or $\mathbb{1}$ (all bits are zero except the least significant bit (LSB)). 
So, for a given ciphertext $c$, the decrypted message $m=\mathbb{0}/\mathbb{1}$ is fully depends on the secret coefficient $\Bar{\bf s}_{0}[0]$. In the paper ~\cite{Sidechannelattacks1}, the distinguisher $\mathcal{O}$ called binary PC oracle defines as follows 
 \begin{equation}
{\mathcal{O}}(c)=
    \begin{cases}
        0 & \text{if } \text{PKE\_Dec}( c)=\mathbb{0}\\
        1 & \text{if } \text{PKE\_Dec}( c)=\mathbb{1}
    \end{cases}
\end{equation}
to distinguish $m=\mathbb{0}/\mathbb{1}$ by the EM power analysis. Since $\Bar{\bf s}_{0}[0]$ directly depends on the message $m$, using the binary plaintext checking oracle, the attacker gets a bit of information of the coefficient $\Bar{\bf s}_{0}[0]$. Depending on this information, the attacker creates another ciphertext to query and gets another bit of information. So basically, the attacker has a decision-making binary tree such that using this tree, they construct the next ciphertext and ultimately find the secret coefficient $\Bar{\bf s}_{0}[0]$. 


%In the paper \cite{Sidechannelattacks1}, the authors present generic and practical EM side-channel assisted chosen-ciphertext attacks applicable to six IND-CCA secure LWE/LWR-based PKE/KEMs. These schemes were the candidates in the NIST standardization process. They demonstrate very efficient strategies to instantiate the EM side-channel as two particular plaintexts checking oracle $\mathcal{O}$ as follows:
 %   \begin{equation}
%{\mathcal{O}}(c)=
 \iffalse
 
 \begin{cases}
        0 & \text{if } dec( c)=\text{ all zero}\\
        1 & \text{if } dec( c)=\text{ all zero except least message bit}
    \end{cases}
\end{equation}\\
    They demonstrate their chosen ciphertext attack on the latticed-based post-quantum scheme KYBER \cite{KYBER} and FRODO \cite{FRODO}. They construct the dummy ciphertexts $c$ such that all the coefficient of the decrypted message is zero except the least ($0^{th}$) coefficient and the least coefficient of the decrypted message depends only on one secret coefficient. They describe a  process that helps to find the secret coefficients. To find the secret coefficient $s_{0} [0]$,
they construct the dummy ciphertext $c = (\Bar{\bf u}, {\bf v})$ where $u_{0} [0] = k_{u}$ and $ v[0] = k_{v} $ are non zero and
others coefficients of $\Bar{\bf u}$ and ${\bf v}$ are zero. They choose the value $(k_{u} , k_{v} )$ such that
\begin{equation}
(m)_{j}=
    \begin{cases}
        \text{Decode}(k_{v} - k_{u}s_{0}[0]) & \text{if } j=0\\
        0 & \text{if } 1\leq j\leq n-1
    \end{cases}    
\end{equation}
where Decode() function returns the decrypted message bits of the ciphertext $c$ which depends on the secret coefficient $s_{0}[0]$ and $(k_{u},k_{v}).$ For a fixed $(k_{u},k_{v}),$ the message $m$ depends on only the secret coefficient $s_{0}[0].$ As a result, for various tuples $(k_{u}, k_{v})$, $m = 0$ or $1$ can be utilised as a binary distinguisher $\mathcal{O}$ for each and every potential candidate for $s_{0}[0]$. They create the distinguisher $\mathcal{O}$ to distinguish $m=0$ or $1$ by the EM power analysis.
\fi

By similar construction of ciphertext, they recover the other secret coefficients of $\Bar{\bf s}.$ To recover any secret coefficient $\Bar{\bf s}_{i}[j]$ the attacker constructs the dummy ciphertext $c = (\Bar{\bf u}, {\bf v})$ where $\Bar{\bf u}_{i} [(n-j)\%n] = k_{u}$ and $ {\bf v}[0] = k_{v} $ are non zero and
others coefficients of $\Bar{\bf u}$ and ${\bf v}$ are zero.
Then the decrypted message $m$ will be
\begin{equation}
m^{k}=
    \begin{cases}
        \text{Decode}(k_{v} - (sign)*k_{u}\Bar{\bf s}_{i}[(j+k)\%n]) & \text{if } k=0\\
         \text{Decode}( - (sign)*k_{u}\Bar{\bf s}_{i}[(j+k)\%n]) & \text{if } 1\leq k \leq n-1
    \end{cases}    
\end{equation}
Here the $sign$ is the sign of the $k^{th}$ coefficient of the polynomial $\langle{\bf \Bar{u}},{\bf \Bar{s}}\rangle$. Also. in this case, the attacker selects the value of $(k_{u},k_{v})$ such that all the bits of the decrypted message $m$ will be zero except the LSB. The LSB of the decrypted message will be
\begin{equation}
m^{0}=
    \begin{cases}
        \text{Decode}(k_{v} - k_{u}\Bar{\bf s}_{i}[j]) & \text{if } j=0\\
         \text{Decode}( - k_{u}(-\Bar{\bf s}_{i}[j])) & \text{Otherwise } 
    \end{cases}    
\end{equation}
Similarly, in this case, we observe a direct correlation between the message bit $m^{0}$ and the secret coefficient $\bar{\bf s}_{i}[j]$. Consequently, the recovery process for $\Bar{\bf s}_{0}[0]$ can be applied to retrieve $\Bar{\bf s}_{i}[j]$ (or -$\Bar{\bf s}_{i}[j]$) in a similar manner. The authors have seen that $2k-4k$ queries require to retrieve the complete secret.



\subsection{Multiple-valued plaintext checking Oracle}
In the paper \cite{ParallelPC}, the authors present side-channel attacks on post-quantum KEMs CRYSTAL KYBER~\cite{KYBER}, SABER~\cite{SABER}, FRODO~\cite{frodo_scheme}, NTRU Prime, as well as SIKE~\cite{SIKE} by creating multiple-valued plaintext-checking oracle $\mathcal{O}_{\mu}$.

In the referenced paper \cite{ParallelPC}, the author introduces a method where the attacker can acquire $t$ bits of information regarding the $t$ secret coefficients in a single query instead of obtaining one-bit information per query. We showcase the recovery of $t$ secret coefficients, $\Bar{{\bf s}}_{0}[0],\Bar{{\bf s}}_{0}[1], \dots,\Bar{{\bf s}}_{0}[t-1]$, while employing a similar methodology to recover the remaining coefficients.

To find the secret coefficients $\Bar{\bf s}_{0} [0], s_{i}[1],\dots,\Bar{\bf s}_{i}[t-1]$,
the attacker construct the dummy ciphertext $ c = (\Bar{\bf u}, {\bf v})$where $\Bar{\bf u}_{0} [0] = k_{u}$ is non zero and
others coefficients of $\Bar{\bf u}$ are zero and 
\begin{equation}
{\bf v}[j]=\begin{cases}
        k_{v_{j}} & \forall ~~0\leq j\leq t-1\\
        0 & \text{ Otherwise } 
    \end{cases}.
\end{equation}

Then the decrypted message $m$ will be
\begin{equation}
    m^{j}=
    \begin{cases}
        \text{PKE\_Dec}(k_{v_{j}} - k_{u}\Bar{\bf s}_{0}[j]) & \text{if } 0\leq j\leq t-1\\
        \text{PKE\_Dec}( - k_{u}\Bar{\bf s}_{0}[j]) & \text{if } t\leq j\leq n-1\\\\
    \end{cases}
\end{equation}
Here also, it is clear that for $0\leq j\leq t-1$, $j^{th}$ bit of the decrypted
message $m$ depends on the corresponding secret coefficient  $\Bar{\bf s}_{0}[j]$ and the values $k_{u}$ and $k_{v_{j}}$. The attacker selects $k_{u}, k_{v_{j}}'s$ such that 
They choose the value $(k_{u} , k_{v} )$ such that $\text{PKE\_Dec}( - k_{u}\Bar{\bf s}_{0}[j])$ will be zero for any secret $\Bar{\bf s}_{0}[j]$ and $\text{PKE\_Dec}(k_{v_{j}} - k_{u}\Bar{\bf s}_{0}[j])$  will depend on the corresponding secret $\Bar{\bf s}_{0}[j]$. i.e.,
\begin{equation}
    m^{j}=
    \begin{cases}
        \text{PKE\_Dec}(k_{v_{j}} - k_{u}s_{i}[j]) & \text{if } 0\leq j\leq t-1\\
        0 & \text{Otherwise} 
    \end{cases}
\end{equation}
Therefore every message $m$ will depend on the first $t$ bits.
In the paper \cite{ParallelPC}, the authors create a multiple-valued plaintext checking oracle $\mathcal{O}_{\mu}$ as follows:
\begin{equation}
{\mathcal{O}_{\mu}}( c:m^{(0)},m^{(1)},\dots,m^{(\mu-1)})= r, \text{ if } \text{PKE\_Dec}(c)=m^{(r)}, 0\leq r\leq \mu-1
\end{equation}

The oracle $\mathcal{O}_{\mu}$ takes input $c$ as ciphertext and $\mu$ messages $m^{(0)},m^{(1)},\dots,m^{(\mu-1)}$
 such that the decryption of the ciphertext $c$ is one of the previous messages. They use a multi-classification neural network (NN) to construct the PC-oracle $\mathcal{O}_{\mu}.$ So, the attacker can find the decrypted message of $m$ using the oracle $\mathcal{O}_{\mu}$. As the first $t$ message bits are directly linked to their corresponding secret coefficients, the attacker acquires $t$ bits of information of the coefficients $\Bar{\bf s}{0}[0], \dots, \Bar{\bf s}{0}[t-1]$ using the decrypted message $m$. 

 %Next, the attacker creates the ciphertext with the values $k_{v_{j}}$, which has been selected from the binary decision-making corresponding information of $j^{th}$ bit.   

\iffalse\begin{equation}
    u_{i'}[j]=
    \begin{cases}
        k_{u} & \text{if } i'=i, j=0\\
        0 & \text{ Otherwise } 
    \end{cases}
\text{ and } v[j]=\begin{cases}
        k_{v_{j}} & \forall ~~0\leq j\leq t-1\\
        0 & \text{ Otherwise } 
    \end{cases}.
\end{equation}
They choose the value $(k_{u} , k_{v} )$ such that
\begin{equation}
    (m)_{j}=
    \begin{cases}
        \text{PKE\_Dec}(k_{v_{j}} - k_{u}s_{i}[j]) & \text{if } 0\leq j\leq t-1\\
        0 & \text{Otherwise} 
    \end{cases}
\end{equation}\fi

%Here \text{PKE\_Dec}() function returns the decrypted message bits of the ciphertext $c$ which depends on the secret coefficients $(s_{i} [0], s_{i}[1],\dots,s_{i}[t-1])$ and $(k_{u},k_{v_{0}},k_{v_{1}},\dots,k_{v_{t-1}}).$ For a fixed $(k_{u},k_{v_{0}},k_{v_{1}},\dots,k_{v_{t-1}}),$ the message $m$ depends on only the secret coefficients $(s_{i} [0], s_{i}[1],\dots,s_{i}[t-1]).$ As a result, for various tuples $(k_{u},k_{v_{0}},k_{v_{1}},
%\dots,k_{v_{t-1}})$, $m$ can be utilised as a parallel binary distinguisher $\mathcal{O}_{\mu}$ for each and every potential candidate for $(s_{i} [0], s_{i}[1],\dots,s_{i}[t-1]).$. By similar construction of ciphertext, they recover the other secret coefficients of $\Bar{\bf s}.$ In every query, the attacker collects $t$ bit information. The authors have seen that for Kyber 512, $t=12$, $197$ queries require to retrieve the complete secret. 
%In our research paper, we expanded the parallelization process to enhance secret retrieval by reducing the number of queries. Additionally, we present an approach, leveraging side-channel analysis known as row hammer, to construct our plaintext checking oracle. 

By similar construction of ciphertext, they recover the other secret coefficients of $\Bar{\bf s}.$ In every query, the attacker collects $t$ bit information. The authors have seen that for Kyber 512, $t=12$, $197$ queries require to retrieve the complete secret. 

 One significant area of research in this domain revolves around improving the efficiency of attacks by minimizing the number of required traces. This reduction in traces enables a more precise evaluation of the cost of an optimal attack.
By expanding the parallel plaintext checking oracle technique described in \cite{ParallelPC}, which will lead to fewer queries, we hope to contribute to this goal in this study. Additionally, we will present a practical micro-architectural attack row hammer on the targeted schemes. To accomplish this. We first explain the process of finding the secret key using the extended parallel plaintext checking oracle model introduced in \cite{ParallelPC}. Subsequently, we detail our approach to decrease the number of queries further. The subsequent section outlines the experimental setup for implementing the parallel plaintext checking oracle.
